Recurrent Neural Network Language Model Adaptation Derived Document Vector

In many natural language processing (NLP) tasks, a document is commonly modeled as a bag of words using the term frequency-inverse document frequency (TF-IDF) vector. One major shortcoming of the frequency-based TF-IDF feature vector is that it ignores word orders that carry syntactic and semantic relationships among the words in a document, and they can be important in some NLP tasks such as genre classification. This paper proposes a novel distributed vector representation of a document: a simple recurrent-neural-network language model (RNN-LM) or a long short-term memory RNN language model (LSTM-LM) is first created from all documents in a task; some of the LM parameters are then adapted by each document, and the adapted parameters are vectorized to represent the document. The new document vectors are labeled as DV-RNN and DV-LSTM respectively. We believe that our new document vectors can capture some high-level sequential information in the documents, which other current document representations fail to capture. The new document vectors were evaluated in the genre classification of documents in three corpora: the Brown Corpus, the BNC Baby Corpus and an artificially created Penn Treebank dataset. Their classification performances are compared with the performance of TF-IDF vector and the state-of-the-art distributed memory model of paragraph vector (PV-DM). The results show that DV-LSTM significantly outperforms TF-IDF and PV-DM in most cases, and combinations of the proposed document vectors with TF-IDF or PV-DM may further improve performance.

==> Table/tbl-PVparam_c.tex <==
\begin{table}[tbph]
	\begin{center}
		\vspace{2mm}
		
		\caption{\it The hyperparameter chosen in the test (you can hide this by comment out)}
		
		\begin{tabular}{| c | c | c | c |}
			\hline 
			       & PTB  & Brown & BNC Baby \\
			\hline 
			\hline                       
			window size  & 20 & 15 & 15\\ 
			\hline            
			Min frequency & 5 & 5  &  10 \\ 
			\hline
			negative word samples & 10 & 20 & 10\\
			\hline
			Sub-sampling &0 & 0&0 \\ 
			\hline
		
	%		Vector Dimension & 100 & 500 &2000 \\ 
	%		\hline  
		%	Epoch  & 5 & 10& 20 &-   \\ 
			%\hline
		\end{tabular}
		
		\label{tbl:hyperpara_c}
	\end{center}	 
\end{table}	

==> Table/tbl-brown.tex <==
\begin{table}[tbph]
  \begin{center}
    \caption{\it Genre classification accuracy (\%). The baseline result labeled with * is quoted from \cite{wu2010fine}.}
    \vspace{2mm}

    \begin{tabular}{| c | c | c | c | c | c | c |} \hline
      Features &Penn Treebank  & Brown & BNC Baby  \\
      \hline \hline
			
      4-char-gram* & 64.40 &&\\ 
      \hline
  %    1-gram, $\z$ &   &   &   \\
 %     3-gram, $\z$ &    &  &   \\ 
      5-gram, $\z_5$ &   &  &   \\ 
      %Brown Clustering, $\c$ &   & 0.797011 (+/- 0.165478)  &   \\ 
      $PV_{500}$ &  &  & 98.35  \\ 
      %$PV_{500}$-$\z$ &  64.47 (+/- 0.90)  &  75.72 (+/- 1.04) & \bf 99.63 (+/- 0.26)   \\     			
      \hline
			
      $\h$  & 0.606600 (+/- 0.117991) & 0.781123 (+/- 0.160753) & 0.986287 (+/- 0.054532) \\ 
      $\h$-$\k$  & 0.606000 (+/- 0.116550) & 0.849783 (+/- 0.125865) & 0.982982 (+/- 0.059519)  \\ 
    %  \hline
%      $\h$-$\k$-$PV_{500}$ & & &   \\
      $\h$-$\z_5$ & 0.781123 (+/- 0.160753) & 0.868188 (+/- 0.131495) & 0.993947 (+/- 0.034441) \\ % 
      \hline

    
      $\b_{m_{100}}$  & 0.600800 (+/- 0.115089) & 0.760127 (+/- 0.180845) & 0.989035 (+/- 0.043874) \\
      %$\b_l$  && & \\
      $\b_{c_{100}}$  & 0.638800 (+/- 0.130577) & 0.820109 (+/- 0.142445) & 0.994532 (+/- 0.032818) \\
      $\d_{m_{100}}$  & 0.651200 (+/- 0.109152) & 0.851232 (+/- 0.143622) & 1 \\ 
      \hline
       $\d_m$-$PV_{500}$& 0.671600 (+/- 0.119490) & 0.875942 (+/- 0.123864) & 1 \\ 
       $\d_m$-$\z_5$  &0.663600 (+/- 0.119248) & 0.871866 (+/- 0.118578)& 1 \\
       \hline
      
      $\b_{m_{250}}$  & &  & 98.91 \\
      $\b_{c_{250}}$  & &   & 99.83 \\
      $\d_{m_{250}}$  &0.597600 (+/- 0.132457) & 0.841812 (+/- 0.121212)  & 0.993450 (+/- 0.035486) \\ 
      \hline

  
     
    \end{tabular}
    
    \label{tbl:results.accuracy}
  \end{center}
\end{table}


==> Table/tbl-lr.tex <==
\begin{table}[tbph]
  \begin{center}
    \vspace{2mm}

    \caption{\it The initial learning rate used in the DV-LSTM and DV-RNN adaptation.}
      \begin{tabular}{|c|c|c|c|}
         \hline
              Models & PTB  &  Brown & BNC \\ \hline
           \hline 
            DV-RNN&0.1 &0.1 &0.1 \\ \hline
            DV-LSTM-100& 0.05 & 0.02 & 0.02 \\ \hline
	        DV-LSTM-250& 0.1 &0.05 & 0.05  \\ \hline
    \end{tabular}
    	    
    \label{tbl:lr}
  \end{center}	 
\end{table}	

==> Table/tbl-results-accuracy.tex <==
\begin{table}[tbph]
  \begin{center}
    \caption{\it Genre classification accuracy (\%). %The baseline result labeled with * is quoted from \cite{wu2010fine}.
    }
    \vspace{2mm}

    \begin{tabular}{| c | c | c | c | c | c | c |} \hline
      Features& PTB & Brown & BNC Baby  \\
      \hline \hline
			
      4-char-gram* & 64.40 &-&-\\   \hline
	5-gram, $\z_5$ &80.91&65.24&96.27 \\ \hline
	$\c_{500}$ &79.70&62.92&94.51 \\ 	\hline
	$PV_{500}$ &81.63&\bf65.68&98.35 \\ \hline
	\hline
	$\d_{m_{100}}$ &75.93&60.14&98.50 \\ \hline
	$\b_{c_{100}}$ &82.63&63.88&99.45 \\ \hline
	$\d_{m_{100}}$ &\bf84.70&65.20&\bf100.00 \\ \hline
	$d_{m_{100}}$-$PV_{500}$ &86.00&\bf67.00&\bf100.00 \\ \hline
	$\d_{m_{100}}$-$\z^{1000}_5$ &\bf 86.38&66.84&\bf100.00 \\ \hline
%	\hline
%	$\b_{m_{250}}$ &73.80&60.04&98.91 \\ \hline
%	$\b_{c_{250}}$ &82.30&63.26&99.83 \\ \hline
%	$\d_{m_{250}}$ &\bf84.89&\bf66.46&99.67 \\ \hline
%	X_lstm250_d2vnom &84.61&66.22&99.95 \hline
%	X_lstm250_bow &85.70&66.34&100.00 \hline
%	\hline
%	$\h$-$\k$ &85.48&60.66&98.30 \\ \hline
%	$\h$ &78.11&55.12&98.63 \\ \hline
%	$\k$ &79.29&60.22&97.85 \\ \hline
%	$\h$-$\z_5$  &86.82&65.80&99.39 \\ \hline
%	$\h$-$\z_5$  &87.27&65.62&99.39 \\ \hline
  
    \end{tabular}
    
    \label{tbl:results.accuracy}
  \end{center}
\end{table}


==> Table/tbl-results-rnnlm-a.tex <==
\begin{table}[tbph]
  \begin{center}
    \caption{\it Genre classification accuracy of DV-RNN (\%).}
    \vspace{2mm}

    \begin{tabular}{| c | c | c | c | c | c | c |} \hline
      Features& PTB & Brown & BNC Baby  \\
      \hline \hline
	\hline
	$\h$-$\k$ &85.48&60.66&98.30 \\ \hline
	$\h$ &78.11&55.12&98.63 \\ \hline
	$\k$ &79.29&60.22&97.85 \\ \hline
	$\h$-$\z_5$  &\bf 86.82&65.80&\bf 99.39 \\ \hline
%	$\h$-$\z_5$  &87.27&65.62&99.39 \\ \hline
  
     
    \end{tabular}
    
    \label{tbl:results.accuracy.rnn}
  \end{center}
\end{table}


==> Table/tbl-results-ttest.tex <==
\begin{table}[tbph]
  \begin{center}
    \caption{\it T-test score, baseline is always PV. So every score here is the DV-L100-LSTM100 or DV-LSTM250 compared with $PV_{500}$ ('acc' stands for accuracy, fs stands for f-score. 2.262 is the 0.95 confidence threshold, 3.250 is the 0.99 confidence threshold,3.690 is the 0.995 threshold, 4.781 is the 0.999 threshold, that is when ttest score> threshold, we reject the null hypothesis and claim the data has significant difference. Therefore, basically we can claim 0.995 confidence.)
    %The baseline results labeled with * are quoted from \cite{tang2015automatic}.
    }
    \vspace{2mm}
      \begin{tabular}{| c | c | c | c | c |} \hline
      	Features & PTB  & Brown & BNC Baby  \\
      	\hline \hline
      
  
	$\d_{m_{100}-acc}$  & 7.8209 &0.6560&62.9813 \\ \hline
	$\d_{m_{100}-fs}$  &6.6864 &0.0325& 359.8413 \\ \hline
	$\d_{m_{250}-acc}$ &7.2670 & 3.73836222331 &13.2364\\ \hline
	$\d_{m_{250}-fs}$ & 6.8028 & 4.1253458168 &12.8700\\ \hline
	$\h$-$\z_5$-acc & 16.5029 & - & 18.2335\\ \hline
	$\h$-$\z_5$-fs & 16.7453 & - & 16.1958\\ \hline
	18.23345
	
    
      \end{tabular}

    \label{tbl:results.ttest}
  \end{center}
\end{table}

